Boosting End-to-End Database Isolation Checking via Mini-Transactions (Extended Version)

Transactional isolation guarantees are crucial for database correctness. However, recent studies have uncovered numerous isolation bugs in production databases. The common black-box approach to isolation checking stresses databases with large, concurrent, randomized transaction workloads and verifies whether the resulting execution histories satisfy specified isolation levels. For strong isolation levels such as strict serializability, serializability, and snapshot isolation, this approach often incurs significant end-to-end checking overhead during both history generation and verification. We address these inefficiencies through the novel design of Mini-Transactions (MTs). MTs are compact, short transactions that execute much faster than general workloads, reducing overhead during history generation by minimizing database blocking and transaction retries. By leveraging MTs' read-modify-write pattern, we develop highly efficient algorithms to verify strong isolation levels in linear or quadratic time. Despite their simplicity, MTs are semantically rich and effectively capture common isolation anomalies described in the literature. We implement our verification algorithms and an MT workload generator in a tool called MTC. Experimental results show that MTC outperforms state-of-the-art tools in both history generation and verification. Moreover, MTC can detect bugs across various isolation levels in production databases while maintaining the effectiveness of randomized testing with general workloads, making it a cost-effective solution for black-box isolation checking.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> figs/alg/divergence.tex <==
% divergence.tex

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width = 0.55\textwidth]{figs/fork}
		\caption{The \exception{} pattern: transactions $T_{2}$ and $T_{3}$ read the same value of $x$
		  from $T_{1}$ and then write different values.}
		\label{fig:pattern}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width = 0.65\textwidth]{figs/fork-existence}
		\caption{Transactions $T_{a}$ and $T_{c'}$ read the same value of $x$
		  from $T_{a'}$ and then write different values.}
		\label{fig:pattern-existence}
	\end{subfigure}
	\caption{Illustration of the \exception{} pattern
	  (\protect\subref{fig:pattern})
	  and the proof of Lemma~\ref{lemma:acyclic-implies-total}
		(\protect\subref{fig:pattern-existence}).}
	\label{fig:ser-proof}
\end{figure}

==> figs/bug-detection/bug-detection.tex <==
% bug-detection.tex

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width = 1.00\textwidth]{figs/bug-detection/pg-time}
		\caption{Time}
		\label{fig:pg-time}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.24\textwidth}
		\centering
		\includegraphics[width = 1.00\textwidth]{figs/bug-detection/pg-abort-rate}
		\caption{Abort rate}
		\label{fig:pg-abort-rate}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.28\textwidth}
		\centering
		\includegraphics[width = 1.00\textwidth]{figs/bug-detection/pg-bug}
		\caption{Number of bugs detected}
		\label{fig:pg-bug}
	\end{subfigure}

	% \vspace{5pt}
	% \begin{subfigure}[b]{0.20\textwidth}
	% 	\centering
	% 	\includegraphics[width = 1.00\textwidth]{figs/bug-detection/mongo-time}
	% 	\caption{Time}
	% 	\label{fig:mongo-time}
	% \end{subfigure}
	% \hfill
	% \begin{subfigure}[b]{0.20\textwidth}
	% 	\centering
	% 	\includegraphics[width = 1.00\textwidth]{figs/bug-detection/mongo-abort-rate}
	% 	\caption{Abort rate}
	% 	\label{fig:mongo-abort-rate}
	% \end{subfigure}
	% \hfill
	% \begin{subfigure}[b]{0.28\textwidth}
	% 	\centering
	% 	\includegraphics[width = 1.00\textwidth]{figs/bug-detection/mongo-bug}
	% 	\caption{Bugs detected}
	% 	\label{fig:mongo-bug}
	% \end{subfigure}
	\caption{Effectiveness of \ourtool in detecting isolation bugs.}
	\label{fig:bug-detection}
\end{figure}

==> figs/comp-exp/ser-e2e-time-memory-4subfigs-tex.tex <==
% ser-e2e-time-memory-4subfigs-tex.tex

\begin{figure*}[t]
	\centering
	\includegraphics[width = 0.75\textwidth]{figs/comp-exp/ser-e2e-time-memory-4subfigs}
	\caption{End-to-end checking performance,
	  with time decomposed into history generation and verification.}
	\label{fig:ser-e2e-time-memory-4subfigs}
\end{figure*}

==> figs/comp-exp/ser-validation-e2e.tex <==
% ser-validation-e2e.tex

\usetikzlibrary{patterns}
\begin{figure*}[h]
	\centering
	\resizebox{.8\linewidth}{!}{
		\begin{tikzpicture}
			\centering
			\begin{axis}[
					hide axis,
					width=2cm, % Set width to minimum (1pt)
					height=2cm, % Set height to minimum (1pt)
					area legend,
					legend style={at={(1,-0.1)},anchor=south, legend columns=5,draw=none},
					/tikz/every even column/.append style={column sep=0.5cm}
				]
				\addlegendimage{color=red, pattern color=red, pattern=crosshatch}
				\addlegendentry{\footnotesize \ourtool gen}
				\addlegendimage{color=blue, pattern color=blue}
				\addlegendentry{\footnotesize Cobra gen}
				\addlegendimage{color=red, fill=red}
				\addlegendentry{\footnotesize \sertool}
				\addlegendimage{color=blue, pattern color=blue, pattern=crosshatch dots}
				\addlegendentry{\footnotesize Cobra  w/o GPU}
				\addlegendimage{color=blue, pattern color=blue, pattern=horizontal lines}
				\addlegendentry{\footnotesize Cobra  w/ GPU}
				\addplot[draw=none] coordinates {(0,0)}; % Dummy plot for reference
			\end{axis}
		\end{tikzpicture}
	}

	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width = \textwidth]{figs/comp-exp/ser-e2e-txns.pdf}
	%	\caption{time against \#txns, e2e}
	\caption{}
		\label{fig:ser-validation-e2e-txns}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width = \textwidth]{figs/comp-exp/ser-e2e-ops.pdf}
	%	\caption{time against \#ops, e2e}
	\caption{}
		\label{fig:ser-validation-e2e-ops}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width = \textwidth]{figs/comp-exp/ser-e2e-keys.pdf}
		%	\caption{time against \#objects, e2e}
		\caption{}
		\label{fig:ser-validation-e2e-keys}
	\end{subfigure}
	\caption{End-to-end checking time for SER,
	  decomposed into history generation and verification.}
	\label{fig:ser-validation-e2e}
\end{figure*}

==> figs/ser.tex <==
% \pgfplotstableread[col sep=comma]{sim.csv}\datatable
\begin{figure*}
\pgfplotstableread{
    50 1 2.92 4.04
    100 1 3.625 3.46875
    200 1 2.81578947368421 4.57894736842105
    500 1 1.77611940298507 7.80597014925373
    1000 1 1.57522123893805 33.1769911504425
    1500 1 1.22916666666667 91.7864583333333
    2000 1 1.27619047619048 231.052380952381
}{\datatable}

\begin{tikzpicture}
    \begin{axis}[
        ybar,
        ylabel=Normalized Time Cost,
        xlabel=\# of Txns,
        ymin=0,
        log origin y=infty,
        xtick=data,
        xticklabels from table={\datatable}{0},
        bar width=0.2cm,
        legend style={at={(0.25,0.7)},anchor=south},
        ymode=log
        % scaled y ticks=manual:{}{\pgfmathparse{#1>10 ? ln(#1) : #1}}
    ]
    \addplot table [x expr=\coordindex, y index=1] {\datatable};
    \addlegendentry{lwt}
    \addplot table [x expr=\coordindex, y index=2] {\datatable};
    \addlegendentry{cobra(w GPU)}
    \addplot table [x expr=\coordindex, y index=3] {\datatable};
    \addlegendentry{cobra(w/o GPU)}
    \end{axis}
    \end{tikzpicture}
    \label{fig:ser}
\end{figure*}

==> sections/proof.tex <==
% proof.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness Proofs}
\label{ss:proofs}

\input{figs/alg/pattern-existence}

In this section, we provide correctness proofs,
which are surprisingly intricate,
for the three verification algorithms
in Algorithm~\ref{alg:mini-checking}.

%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:no-fork-implies-total}
	If the graph $\G$ returned by \emph{\consdep}
	does not contain any $\WW$ loops or
	any instances of the \exception{} pattern,
	then it is a dependency graph of $\H$.
\end{lemma}



\begin{proof} \label{proof:no-fork-implies-total}
	Suppose that $\G$ does not contain any $\WW$ loops or
	any instances of the \exception{} pattern.
	We need to show that for each object $k \in \Key$,
	$\WW(k)$ is a strict total order on the set $\WriteTx_{x}$.
	Suppose by contradiction that
	there exists an object $x \in \Key$
	such that $\WW(x)$ is not a strict total order on $\WriteTx_{x}$.
	In the following, we identify an instance of the \exception{} pattern in $\G$.
	% We claim that there must be three transactions $T_{1}$, $T_{2}$, and $T_{3}$ in $\H$
	% such that
	% \begin{inparaenum}
	% 	\item $T_{2}$ and $T_{3}$ read the same value of $x$ from $T_{1}$
	% 		and then write different values to $x$, and
	% 	\item there are no $\WW(x)$ dependency edges between $T_{2}$ and $T_{3}$ in $\G$.
	% \end{inparaenum}
	% This is illustrated in Figure~\ref{fig:pattern}.

	Since $\G$ does not contain any $\WW$ loops,
	$\WW(x)$ is a strict order.
	Therefore, $\WW(x)$ is not total.
	Consider two transactions $T_{a}$ and $T_{b}$
	such that they both write to $x$ with different values,
	but there are no $\WW(x)$ dependency edges between them in $\G$;
	see Figure~\ref{fig:pattern-existence}.
	If $T_{a}$ and $T_{b}$ read the value of $x$ from the same transaction,
	then we are done.
	Otherwise, consider the transactions $T_{a'}$ and $T_{b'}$
	($T_{a'} \neq T_{b'}$) from which
	$T_{a}$ and $T_{b}$ read the value of $x$, respectively.
	That is, $T_{a'} \rel{\WR(x)/\WW(x)} T_{a}$ and
	$T_{b'} \rel{\WR(x)/\WW(x)} T_{b}$
	(see line~\ref{line:ww-edges} of \consdep).
	It is clear that $T_{a'} \neq T_{b}$ and $T_{b'} \neq T_{a}$,
	since otherwise there would be a $\WW(x)$ dependency edge between $T_{a}$ and $T_{b}$.
	There are two cases regarding whether there is a $\WW(x)$ dependency edge
	between $T_{a'}$ and $T_{b'}$ in $\G$:
	\begin{itemize}
		\item Suppose there is a $\WW(x)$ dependency edge between $T_{a'}$ and $T_{b'}$ in $\G$,
			say $T_{a'} \rel{\WW(x)} T_{b'}$.
			Note that this $\WW(x)$ edge may be derived by transitivity
			(see line~\ref{line:ww-tc} of \consdep).
			Let $T_{c'}$ be a transaction \emph{directly following} $T_{a'}$
			in the $\WW(x)$ dependency chain from $T_{a'}$ to $T_{b'}$.
			That is, the edge $T_{a'} \rel{\WW(x)} T_{c'}$
			coincides with $T_{a'} \rel{\WR(x)} T_{b'}$
			(see line~\ref{line:ww-edges} of \consdep).
			As illustrated in Figure~\ref{fig:pattern-existence},
			we have $T_{a'} \rel{\WR(x)/\WW(x)} T_{c'} \rel{\WW(x)} T_{b'}$.
			It is possible that $T_{c'} = T_{b'}$, but we argue that
			\begin{itemize}
				\item $T_{c'} \neq T_{a}$.
				  Otherwise, we have $T_{a} = T_{c'} \rel{\WW(x)} T_{b'} \rel{\WW(x)} T_{b}$.
					Then by transitivity, $T_{a} \rel{\WW(x)} T_{b}$,
					contraditing the assumption that there is no $\WW(x)$ dependency edge
					between $T_{a}$ and $T_{b}$.
				\item $T_{c'} \neq T_{b}$.
				  Otherwise, we have $T_{b} = T_{c'} \rel{\WW(x)} T_{b'} \rel{\WW(x)} T_{b}$.
					Then by transitivity, $T_{b} \rel{\WW(x)} T_{b}$,
					contraditing the assumption that $\G$ contains no $\WW(x)$ loops.
			\end{itemize}

			Therefore, $T_{a'}$, $T_{c'}$, and $T_{a}$ forms an instance
			of the \exception{} pattern.
		\item If there is no a $\WW(x)$ dependency edge
			between $T_{a'}$ and $T_{b'}$ in $\G$,
			we apply the same argument above to $T_{a'}$ and $T_{b'}$.
	\end{itemize}
	Since the number of transactions in $\H$ is finite
	and $\H$ contains an initial transaction $\bot_{T}$
	which install initial values to all objects,
	we will eventually identify three transactions
	that form an instance of the \exception{} pattern.
\end{proof}
%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:acyclic-implies-total}
	If the graph $\G$ returned by \emph{\consdep} is acyclic,
	then it is a dependency graph of $\H$.
\end{lemma}

\begin{proof} \label{proof:fork}
	Suppose by contradiction that $\G$ is not a dependency graph of $\H$.
	By Lemma~\ref{lemma:no-fork-implies-total},
	$\G$ contains $\WW$ loops or instances of the \exception{} pattern.
	Since $\G$ is acyclic, there are no $\WW$ loops in $\G$.
	Thus, $\G$ must contain instances of the \exception{} pattern,
	as illustrated in Figure~\ref{fig:pattern}.
	However, in this case, there would be a cycle
	$T_{2} \rel{\RW(x)} T_{3} \rel{\RW(x)} T_{2}$ in $\G$.
\end{proof}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\begin{theorem}[Correctness of \checksser]
	\label{thm:correctness-checksser}
	\checksser{} returns \true{} if and only if $\H$ satisfies \sser.
\end{theorem}

\begin{proof} \label{proof:correctness-checksser}
	The proof proceeds in two directions.

%	\begin{itemize}
	%	\item 
	``$\implies$'': 
		  Suppose that \checksser{} returns \true.
			Then the graph $\G$ at line~\ref{line:checksser-call-consdep}
			of \checksser{} is acyclic.
		  By Lemma~\ref{lemma:acyclic-implies-total},
			$\G$ is a dependency graph of $\H$.
			By Definition~\ref{def:sser},
			$\H$ satisfies \sser.
	
	%	\item 
	``$\;\Longleftarrow\;$'':
		  Suppose that \checksser{} returns \false.
			Then the graph $\G$ at line~\ref{line:checksser-call-consdep}
			of \checksser{} is cyclic.
			Since $\G$ is a subgraph of any dependency graph of $\H$,
			no dependency graph of $\H$ is acyclic.
			By Definition~\ref{def:sser},
			$\H$ does not satisfy \sser.
%	\end{itemize}
\end{proof}
%%%%%%%%%%%%%%%

Similarly, by Lemma~\ref{lemma:acyclic-implies-total} and Definition~\ref{def:ser},
we can establish the correctness of \checkser{}.
The proof is omitted here.

%%%%%%%%%%%%%%%
\begin{theorem}[Correctness of \checkser]
	\label{thm:correctness-checkser}
	\checkser{} returns \true{} if and only if $\H$ satisfies \ser.
\end{theorem}

% \begin{proof} \label{proof:correctness-checkser}
% 	The proof proceeds in two directions.
% 	\begin{itemize}
% 		\item (``$\implies$'')
% 		  Suppose that \checkser{} returns \true.
% 			Then the graph $\G$ at line~\ref{line:checkser-call-consdep}
%				of \checkser{} is acyclic.
% 		  By Lemma~\ref{lemma:acyclic-implies-total},
% 			$\G$ is a dependency graph of $\H$.
% 			By Definition~\ref{def:ser},
% 			$\H$ satisfies serializability.
% 		\item (``$\;\Longleftarrow\;$'')
% 		  Suppose that \checkser{} returns \false.
% 			Then the graph $\G$ at line~\ref{line:checkser-call-consdep}
%				of \checkser{} is cyclic.
% 			Since $\G$ is a {subgraph} of any dependency graph of $\H$,
% 			no dependency graph of $\H$ is acyclic.
% 			By Definition~\ref{def:ser},
% 			$\H$ does not satisfy serializability.
% 	\end{itemize}
% \end{proof}
%%%%%%%%%%%%%%%

Finally, we show the correctness of \checksi{}.
%%%%%%%%%%%%%%%
\begin{theorem}[Correctness of \checksi]
	\label{thm:correctness-checksi}
	\checksi{} returns \true{} if and only if $\H$ satisfies \si.
\end{theorem}

	% A mini-transaction history satisifes snapshot isolation if and only if
	% its dependency graph contains only cycles (if any) with at least two adjacent $\RW$ edges.

\begin{proof} \label{proof:si-theorem-mini}
	The proof proceeds in two directions.
	
%	\begin{itemize}
	%	\item 
	``$\;\Longleftarrow\;$'':
		  We show that if \checksi{} returns \false,
			then $\H$ does not satisfy SI.
		  There are two cases:
			\begin{itemize}
				\item Suppose that \checksi{} returns \false{}
				at line~\ref{line:checksi-return-false} of \checksi.
				Then $\G$ contains an instance of the \exception{} pattern.
				By Lemma~\ref{lemma:fork-violates-si},
				$\H$ does not satisfy SI.
				\item Suppose that \checksi{} returns \false{}
				at line~\ref{line:checksi-acyclic} of \checksi.
				There are two cases regarding whether $\G$ contains a $\WW$ loop:
				\begin{itemize}
					\item If $\G'$ contains a $\WW$ loop,
					  then, by the construction of $\G'$
						(line~\ref{line:checksi-g-prime} of \checksi),
						the graph $\G$ at line~\ref{line:checksi-g-prime}
						also contains a $\WW$ loop.
						Since $\G$ is a {subgraph} of any dependency graph of $\H$,
						$\H$ does not admit any {legal} dependency graphs.
						By Definition~\ref{def:si},
						$\H$ does not satisfy SI.
					\item If $\G'$ contains no $\WW$ loops,
					  then, by the construction of $\G'$
						(line~\ref{line:checksi-g-prime} of \checksi),
						$\G$ does not contain any $\WW$ loop either.
						On the other hand, the graph $\G$ at line~\ref{line:checksi-g-prime}
						does not contain any instances of the \exception{} pattern.
						By Lemma~\ref{lemma:no-fork-implies-total},
						the graph $\G$ at line~\ref{line:checksi-g-prime} is a dependency graph of $\H$.
						Since $\G$ is a {subgraph} of any dependency graph of $\H$,
						$\G$ is the {unique} dependency graph of $\H$.
						Then by Definition~\ref{def:si},
						$\H$ does not satisfy SI.
				\end{itemize}
			\end{itemize}
	%	\item 
	
	``$\implies$'':
			If \checksi{} returns \true{}
			at line~\ref{line:checksi-acyclic} of \checksi,
			then $\G'$ at line~\ref{line:checksi-g-prime} of \checksi{} is acyclic.
			Therefore, $\G'$ contains no $\WW$ loops.
			By the line of reasoning above,
			$\G$ at line~\ref{line:checksi-g-prime} is a dependency graph of $\H$.
			Therefore, by Definition~\ref{def:si}, $\H$ satisfies SI.
%	\end{itemize}
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/si-validation-e2e.tex <==
% si-validation-e2e.tex

% \begin{figure*}
% 	\centering
% 	\resizebox{.5\linewidth}{!}{
% 		\begin{tikzpicture}
% 			\centering
% 			\begin{axis}[
% 					hide axis,
% 					width=2cm, % Set width to minimum (1pt)
% 					height=2cm, % Set height to minimum (1pt)
% 					area legend,
% 					legend style={at={(1,-0.1)},anchor=south, legend columns=4,draw=none},
% 					/tikz/every even column/.append style={column sep=0.5cm}
% 				]
% 				\addlegendimage{color=red, pattern color=red, pattern=crosshatch}
% 				\addlegendentry{\footnotesize \ourtool gen}
% 				\addlegendimage{color=blue, pattern color=blue}
% 				\addlegendentry{\footnotesize PolySI gen}
% 				\addlegendimage{color=red, fill=red}
% 				\addlegendentry{\footnotesize \sitool}
% 				\addlegendimage{color=blue, pattern color=blue, pattern=crosshatch dots}
% 				\addlegendentry{\footnotesize PolySI}
% 				\addplot[draw=none] coordinates {(0,0)}; % Dummy plot for reference
% 			\end{axis}
% 		\end{tikzpicture}
% 	}

% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\centering
% 		\includegraphics[width = \textwidth]{figs/comp-exp/si-e2e-txns.pdf}
% 	%	\caption{time against \#txns, e2e}
% 	\caption{}
% 		\label{fig:si-validation-e2e-txns}
% 	\end{subfigure}
% 		\hfill
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\centering
% 		\includegraphics[width = \textwidth]{figs/comp-exp/si-e2e-ops.pdf}
% 		%	\caption{time against \#ops, e2e}
% 		\caption{}
% 		\label{fig:si-validation-e2e-ops}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.32\textwidth}
% 		\centering
% 		\includegraphics[width = \textwidth]{figs/comp-exp/si-e2e-keys.pdf}
% 	%	\caption{time against \#objects, e2e}
% 	\caption{}
% 		\label{fig:si-validation-e2e-keys}
% 	\end{subfigure}
% 	%	\hfill
% 	%	\begin{subfigure}[b]{0.2\textwidth}
% 	%	\centering
% 	%	\includegraphics[width = \textwidth]{figs/mm.jpeg}
% 	%	\caption{XX bug found in YY}
% 	%	\label{xx}
% 	%  \end{subfigure}
% 	\caption{End-to-end checking time for SI,
% 	  decomposed into history generation and verification.}
% 	\label{fig:si-validation-e2e}
% \end{figure*}

==> table/axioms.tex <==
% axioms.tex

\begin{table*}[tbp]
  \centering
  \caption{Consistency axioms, constraining an abstract execution $(\h, \VIS, \AR)$.
    (Adapted from~\protect\cite{AnalysingSI:JACM2018})}
  \label{table:axioms}
  \renewcommand{\arraystretch}{1.3}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|c|}
    \hline
    \multicolumn{3}{|c|}{
	  $\begin{aligned}[c]
		&\forall (\E, \po) \in \h.\;
		  \forall \evar \in \Event.\;
		    \forall \keyvar, \valvar.\;
			  \big(\op(\evar) = \readevent(\keyvar, \valvar)
			  \land \set{\fvar \mid (\op(\fvar) = \_(\keyvar, \_) \land \fvar \rel{\po} \evar} \neq \emptyset\big) \\
			  &\quad \implies \op(\max_{\po} \set{\fvar \mid \op(\fvar) = \_(\keyvar, \_) \land \fvar \rel{\po} \evar}) = \_(\keyvar, \valvar)
	   \end{aligned}$ \hfill (\intaxiom)} \\ \hline
    \multicolumn{3}{|c|}{
	  $\begin{aligned}[c]
		\forall T \in \h.\; \forall \keyvar, \valvar.\; T \vdash \readevent(\keyvar, \valvar) \implies
		  \max_{\AR}(\VIS^{-1}(T) \cap \WriteTx_{\keyvar}) \vdash \writeevent(\keyvar, \valvar)
	  \end{aligned}$ \hfill (\extaxiom)} \\ \hline
    $\SO \subseteq \VIS$ \hfill (\sessionaxiom)
	& $\AR \comp \VIS \subseteq \VIS$ \hfill (\prefixaxiom)
	& $\RT \subseteq \VIS$ \hfill (\rtaxiom) \\ \hline
	$\VIS = \AR$ \hfill (\totalvisaxiom)
	& \multicolumn{2}{c|}{
	$\forall S, T \in \T.\; S \conflict T \implies (S \rel{\VIS} T \lor T \rel{\VIS} S)$
	  \hfill (\noconflictaxiom)} \\ \hline
    \end{tabular}%
  }
\end{table*}
    %   $\forall S, T \in \h.\; S \rel{\VIS} T \implies \starttime(T) > \committime(S)$

==> table/mini-transactions.tex <==
% mini-transactions.tex

\begin{table}[t]
	\centering
	\caption{A survey on mini-transactions.}
	\label{table:mini-transactions}
	\renewcommand\arraystretch{1.2}
	\resizebox{0.85\columnwidth}{!}{%
	\begin{tabular}{|c|c|c|}
		\hline
		{\bf Mini-transactions} & {\bf Databases} & {\bf Isolation Level}  \\ \hline
		Counter & & SSER \\ \hline
		Select for Update & & \\ \hline
		RMW & & \\ \hline
		CAS & & \\ \hline
		Upsert & & \\ \hline
	\end{tabular}}
\end{table}

==> table/new-concurrency.tex <==
\begin{table}[h]
\caption{Concurrency Controlled Results(n=5)}
\label{tbl:new-concurrency}
\centering
\begin{tabular}{|c|c|ll|}
\hline
\multirow{2}{*}{concurrency} & \multirow{2}{*}{nemesis} & \multicolumn{2}{c|}{valid}                              \\ \cline{3-4} 
                             &                          & \multicolumn{1}{c|}{4.2} & \multicolumn{1}{c|}{4.4} \\ \hline
2n                           & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
4n                           & all                      & \multicolumn{1}{l|}{TRUE}  & FALSE                      \\ \hline
6n                           & all                      & \multicolumn{1}{l|}{FALSE}  & TRUE                      \\ \hline
10n                          & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
4n                           & partition                & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
4n                           & kill                     & \multicolumn{1}{l|}{FALSE}  & TRUE                       \\ \hline
4n                           & pause                    & \multicolumn{1}{l|}{TRUE}  & TRUE                      \\ \hline
4n                           & membership               & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
\end{tabular}
\end{table}

==> table/new-rate.tex <==
\begin{table}[h]
\caption{Rate Controlled Results}
\label{tbl:new-rate}
\centering
\begin{tabular}{|c|c|ll|}
\hline
\multirow{2}{*}{rate} & \multirow{2}{*}{nemesis} & \multicolumn{2}{c|}{valid}                              \\ \cline{3-4} 
                      &                          & \multicolumn{1}{c|}{4.2} & \multicolumn{1}{c|}{4.4} \\ \hline
100                   & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
200                   & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
500                   & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
1000                  & all                      & \multicolumn{1}{l|}{TRUE}  & FALSE                       \\ \hline
128                   & partition                & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
128                   & kill                     & \multicolumn{1}{l|}{FALSE} & TRUE                       \\ \hline
128                   & pause                    & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
128                   & membership               & \multicolumn{1}{l|}{TRUE}  & FALSE
\\ \hline
\end{tabular}
\end{table}

==> table/new-timelimit.tex <==
\begin{table}[h]
\caption{Time-limit Controlled Results}
\label{tbl:new-timelimit}
\centering
\begin{tabular}{|c|c|ll|}
\hline
\multirow{2}{*}{time-limit} & \multirow{2}{*}{nemesis} & \multicolumn{2}{c|}{valid}                              \\ \cline{3-4} 
                            &                          & \multicolumn{1}{c|}{4.2} & \multicolumn{1}{c|}{4.4} \\ \hline
100                         & all                      & \multicolumn{1}{l|}{FALSE} & TRUE                       \\ \hline
120                         & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
180                         & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
300                         & all                      & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
60                          & partition                & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
60                          & kill                     & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
60                          & pause                    & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
60                          & membership               & \multicolumn{1}{l|}{TRUE}  & TRUE                       \\ \hline
\end{tabular}
\end{table}

==> table/scylla-exp-config.tex <==
\begin{table}[h]
    \caption{Experimental Setup }
    \label{tbl:scylla-exp-config}
    \centering
    \begin{tabular}{|c|c|}
    \hline
    Component              & Configuration                     \\ \hline
    CPU            & Intel(R) Core(TM) i7-8550U CPU \\ \hline
    Memory              & 4GB                            \\ \hline
    Disk              & 40G                            \\ \hline
    OS            & Ubuntu20.04                    \\ \hline
    Docker            & 20.10.12                       \\ \hline
    Docker-Compose    & 1.25.0                          \\ \hline
    \end{tabular}
    \end{table}
